The Lanczos Approximation for the $\Gamma$-Function with Complex Coefficients

We examined the properties of the coefficients of the \cite{lanczos1964} approximation of the $\Gamma$-function with complex values of the free parameter together with the convergence properties of the approximation when using these coefficients. We report that for fixed real parts of the free parameter that using complex coefficients both increases the computational cost of the Lanczos approximation while drecreasing the accuracy. We conclude that in practical applications of numerical evaluation of the $\Gamma$-function only coefficients generated with real values of the free parameter should be used.

==> Lanczos.tex <==
\section{Method of Lanczos}\label{sec:Lanczos}

\cite{lanczos1964} derived a formula for numerical evaluation of the
\index{Lanczos' Method}
$\Gamma$-function which was popularized to some extent by its inclusion
in \cite{Press1997}. 
It is sufficient to develop the series formula for
the $\Gamma$-function in the right complex half-plane because a numerical
estimate there can be extended to the left complex half-plane by using
the Euler Reflection Formula, Equation \eqref{eqn:reflection}.
\index{Euler Reflection formula}

Lanczos' derivation of his formula proceeds through
three clearly defined phases. The first is to arrive at \cite{lanczos1964}
Equation (11), which is as follows with $r$ being substituted for
Lancozs' symbol $\gamma$. The reasons for this change are explained
below.
\begin{equation}
\Gamma\left(z+\frac{1}{2}\right)=
                   \left(z+r+\frac{1}{2}\right)^{z+\frac{1}{2}}
                   e^{-\left(z+r+\frac{1}{2}\right)}
                   \int_0^e\left[v(1-\log v)\right]^{z-\frac{1}{2}}v^{r}dv.
\label{eqn:Lanczos11}
\end{equation}
Lanczos gave no explanation of how he discovered the usefulness of these
substitutions in developing his series formula. 
\cite{Pugh2004} was able
to simplify the derivation somewhat.

Lanczos started with
\begin{equation}
\Gamma(z+1)=\int_0^{\infty}t^ze^{-t}dt.\label{eqn:Lanczos2}
\end{equation}
In this equation we make the substitution $t\rightarrow\alpha t$ 
($\mathbb{R}e(\alpha)>0$). The limits of the integral are unchanged
and \eqref{eqn:Lanczos2} becomes
$$
\Gamma(z+1)=\alpha^{z+1}\int_0^{\infty}t^ze^{-\alpha t}dt.
$$
If $\alpha$ is real this is an easy substitution. Lanczos does not comment
on the validity for a complex $\alpha$ but \cite{Whittaker1952} assign
the derivation of this substitution in the complex case in Example 2 page
243 of their text.

Lanczos next uses the substition $\alpha=1+\rho z$ but \cite{Pugh2004}
shows that it is quicker to arrive at \eqref{eqn:Lanczos11} by making the
substitution $\alpha=z+\gamma+1$. Note that \cite{Pugh2004} uses the
symbol $r$ in place of $\gamma$ which avoids confusing Lanczos' free
parameter with the Euler-Mascheroni constant. Because this book
contains a significant discussion of the Euler-Mascheroni constant
this change would seem to be helpful in avoiding confusion
so we will use the substitution $\alpha=z+r+1$.
We require that $r \ge 0$.
Then
$$
\Gamma\left(z+1\right)=
 (z+r+1)^{z+1}
 \int_0^{\infty}t^ze^{-(z+r+1)t}dt.
$$
Lanczos now makes the substitutions $t=(1-\log v)$.
The limits of the integration now transform $\infty\rightarrow 0$ and
$0\rightarrow e$ and $dt=-(1/v)dv$. After some algebra we obtain
$$
\Gamma(z+1)=(z+r+1)^{z+1}e^{-(z+r+1)}
            \int_0^e\left[v(1-\log v)\right]^zv^{r}dv.
$$
We now replace $z+1$ by $z+1/2$ to obtain
$$
\Gamma\left(z+\frac{1}{2}\right)=
    \left(z+r+\frac{1}{2}\right)^{z+\frac{1}{2}}
    e^{-\left(z+r +\frac{1}{2}\right)}
            \int_0^e\left[v(1-\log v)\right]^{z-\frac{1}{2}}v^{r}dv
$$
which is \eqref{eqn:Lanczos11}. A plot of the integrand is presented
in Figure (\ref{fig:LanczosFn}).

At this point we can begin to see why the substitutions have yielded
a result which will lend itself to a series expansion. In the integrand
the exponents $z$ and $r$ have been seperated. 

\begin{figure}[ht]
\begin{center}
\includegraphics[width=12cm]{Numerical/LanczosFn.pdf}
\end{center}
\caption{The curve of the integrand in 
Equation \eqref{eqn:Lanczos11}.}
\label{fig:LanczosFn}
\end{figure}

The next phase of the derivation of the series is to transform the integrand
in \eqref{eqn:Lanczos11} into a form to which we can apply Fourier methods.
He first makes the change of variables
\begin{align}
v(1-\log(v))&=1-x^2\label{eqn:Lanczosxtov}
\intertext{which transforms the integral to}
F(z)&=\int_{-1}^1(1-x^2)v^{z-\frac{1}{2}}\frac{dv}{dx}dx \nonumber
\intertext{then undertakes a second change of variables}
x&=\sin\theta \nonumber
\intertext{so that}
F(z)&=\int_{-\pi/2}^{\pi/2}\cos^{2z}\theta f(\theta)d\theta
\label{eqn:LanczosTransform}
\intertext{where}
f(\theta)&=v^r\frac{dv}{\cos\theta d\theta}.\nonumber
\end{align}
The integral \eqref{eqn:LanczosTransform} is sometimes referred to as
the Lanczos Transform.\index{Lanczos Transform}

The actual development of the series is somewhat of a dead-end in 
\cite{lanczos1964} because ultimately he concludes ``the expansion
converges for all values of $z$ in the right half plane, but the convergence
is too slow to be of practical value.'' The point of interest is that
Sterling's series, Equation \eqref{eqn:StirlingAsymptotic}, is 
divergent for all values of $z$ whereas the Lanczos series is
convergent, albeit too slowly in Lanczos' opinion. In fact, the
rate of convergence is slower the closer the value of 
$x$ is to the singularity

To obtain Lanczos' slowly converging series we differentiate 
\eqref{eqn:Lanczosxtov} with respect to $x$ to obtain
\begin{align}
\log v\frac{dv}{dx}&=2x\label{eqn:Lanczosdvdx}.
\intertext{By using \eqref{eqn:Lanczosxtov} again we obtain the
non-linear first order differential equation}
\frac{1}{2}\frac{d}{dx}\left(v^2\right)-(1-x^2)\frac{dv}{dx}-2xv&=0.
\label{eqn:LanczosDE}
\intertext{By inspection of \eqref{eqn:Lanczosxtov} we can see that
for $v$ a function of $x$ that}
v(0)&=1.\label{eqn:LanczosBoundary}
\end{align}
This gives us the single boundary condition necessary to develop
a solution of \eqref{eqn:LanczosDE}.


\cite{lanczos1964} expands $v(x)$ as a Taylor series about $x=0$. The 
function $v(x)$, when treated as a complex of the complex variable $x$ is
analytic within the unit circle $|x|<1$ with a singularity at $x=-1$.
To obtain the coefficients we set
$$
v(x)=1+a_1x+a_2x^2+a_3x^3+\ldots
$$
After  substituting this into \eqref{eqn:LanczosDE}
performing the necessary differentiations and multiplications, we obtain for
the first three terms
\begin{align*}
0&=(a_1^2-2)x+(3a_1a_2-a_1)x^2+(4a_1a_3+2a_2^2)x^3+\ldots
\intertext{Each of the multipliers of the powers of $x$ must be zero. This
allows us to recursively solve for the $a_i$. From the multiplier of $x$}
(a_1^2-2)&=0 \\
   a_1&=\sqrt{2}.
\intertext{Using this value of $a_1$ and  the multiplier of $x^2$ we have}
(3a_1a_2-a_1)&=0 \\
3\sqrt{2}a_2-\sqrt{2}&=0 \\
         a_2&=\frac{1}{3}.
\intertext{Solving for $a_3$}
(4a_1a_3+2a_2^2)=0\\
4\sqrt{2}a_3+2\left(\frac{1}{3}\right)^2&=0  \\
a_3&=-\frac{\sqrt{2}}{36}.
\end{align*}
We can recursively solve for further $a_i$ as necessary.

Let us now return to Equation \eqref{eqn:Lanczos11} which we derived
earlier. We make a (incomplete) change of variable from $v$ to
$\theta$ by setting $\cos^2\theta=v(1-\log v)$. Then the limites of the
integral transform as
\begin{align*}
v=0&\rightarrow \theta=-\frac{\pi}{2} \\
v=e&\rightarrow \theta=\frac{\pi}{2} \\
\end{align*}
Now differentiating the change of variable by $d\theta$ we obtain
\begin{align*}
2\cos\theta\sin\theta&=\log v\frac{dv}{d\theta} 
\intertext{solving for $dv$ we obtain}
dv&=\frac{2\cos\theta\sin\theta d\theta}{\log v}.
\intertext{To simplify our notation we now set}
P_r(z)&=\sqrt{2}\left(z+r+\frac{1}{2}\right)e^{-\left(z+r+\frac{1}{2}\right)}
\intertext{and Equation \eqref{eqn:Lanczos11} can be written}
\Gamma\left(z+\frac{1}{2}\right)&=P_r(z)\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}
          \cos^{2z}\theta\left[\frac{\sqrt{2}v^r\sin\theta}{\log v}\right]
          d\theta.
\end{align*}
We know that we can decompose an arbitrary function into the sum of an even
and an odd function. Thus, denoting the function in the square brackets
by $f_r(\theta)$ then
\begin{align*}
f_r(\theta)=f_{E,r}(\theta)+f_{O,r}(\theta)
\intertext{where}
f_{E,r}(\theta)&=\frac{f_r(\theta)+f_r(-\theta)}{2} \\
f_{O,r}(\theta)&=\frac{f_r(\theta)-f_r(-\theta)}{2} \\
\end{align*}
We now substitute this back into the integral and note that because $\cos$ is
an even function the odd part of $f_r$ integrates to $0$ leaving us 
with
\begin{equation}
\Gamma\left(z+\frac{1}{2}\right)=P_r(z)\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}
          \cos^{2z}\theta f_{E,r}(\theta) d\theta.
\label{eqn:Pugh37}
\end{equation}
At this point Lanczos again takes an excursion in an unproductive direction;
he expands $f_r(\theta)$ in a Taylor series in $\sin\theta$ for
case $r=0$ (Lanczos' $\gamma=0$). This yields a convergent series but
which he declares to be too slow to be of practical significance. 

However, because $f_{E,r}(\theta)$ is an even function it can be expanded
as a Fourier cosine series
\begin{align}
f_{E,r}(\theta)&=\frac{1}{2}a_0(r)+\sum_{k=1}^{\infty}a_k(r)\cos(2k\theta)
\label{eqn:fEvenCosine}
\intertext{where the Fourier coefficients can be obtained from}
a_k(r)&=\frac{2}{\pi}\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}f_{E,r}(\theta)
        \cos(2k\theta)d\theta.\nonumber
\intertext{Let us substitute \eqref{eqn:fEvenCosine} into \eqref{eqn:Pugh37}
to obtain}
\Gamma\left(z+\frac{1}{2}\right)&=P_r(z)\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}
          \cos^{2z}\left[\frac{1}{2}a_0(r)+
          \sum_{k=1}^{\infty}a_k(r)\cos(2k\theta)\right] d\theta\nonumber\\
&=P_r(z)\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}} \cos^{2z}d\theta +
  \sum_{k=1}^{\infty}a_k(r)\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}
        \cos^{2z}\cos(2k\theta)d\theta. \nonumber
\intertext{The values of the integrals can be obtained in closed form 
from}
\int_{-\frac{\pi}{2}}^{\frac{\pi}{2}}\cos^{2z}\cos(2k\theta)d\theta
 &=\sqrt{\pi}\frac{\Gamma\left(z+\frac{1}{2}\right)\Gamma(z+1)}
                  {\Gamma(z+k+1)\Gamma(z-k+1)}. \nonumber
\intertext{With some algebraic manipulation we can obtain the values
of the integral in the following form}
k=0: &=\sqrt{\pi}\frac{\Gamma\left(z+\frac{1}{2}\right)}
                       {\Gamma(z+1)}\nonumber \\
k=1: &=\sqrt{\pi}\frac{\Gamma\left(z+\frac{1}{2}\right)}
                      {\Gamma(z+1)}\left(\frac{z}{z+1}\right)\nonumber \\
k=2: &=\sqrt{\pi}\frac{\Gamma\left(z+\frac{1}{2}\right)}
                      {\Gamma(z+1)}\left(\frac{(z-1)z}{(z+2)(z+1)}\right)
                      \nonumber \\
k=3: &=\sqrt{\pi}\frac{\Gamma\left(z+\frac{1}{2}\right)}
                      {\Gamma(z+1)}
                      \left(\frac{(z-2)(z-1)z}{(z+3)(z+2)(z+1)}\right)
                      \nonumber 
\intertext{Thus \eqref{eqn:Pugh37} can be written}
\Gamma\left(z+\frac{1}{2}\right)&=P_r(z)\sqrt{\pi}
          \frac{\Gamma\left(z+\frac{1}{2}\right)}{\Gamma(z+1)}
   \left[\frac{a_0(r)}{2}+\frac{z}{z+1}a_1(r)+\frac{(z-1)z}{(z+2)(z+1)}a_2(r)
   +\cdots\right]. \nonumber
\end{align}
Now writing out $P_r(z)$ in full, cancelling the term in
$\Gamma\left(z+\frac{1}{2}\right)$ on both sides and multiplying through
by $\Gamma(z+1)$ we obtain
\begin{multline}
\Gamma(z+1)=
\sqrt{2\pi}\left(z+r+\frac{1}{2}\right)^{z+\frac{1}{2}}
             e^{-\left(z+r+\frac{1}{2}\right)} \\
    \left[\frac{a_0(r)}{2}+\frac{z}{z+1}a_1(r)+\frac{(z-1)z}{(z+2)(z+1)}a_2(r)
   +\cdots\right]
\label{eqn:LanczosSeries}
\end{multline}

